Task and Configuration Space Compliance of Continuum Robots via Lie Group and Modal Shape Formulations

Continuum robots suffer large deflections due to internal and external forces. Accurate modeling of their passive compliance is necessary for accurate environmental interaction, especially in scenarios where direct force sensing is not practical. This paper focuses on deriving analytic formulations for the compliance of continuum robots that can be modeled as Kirchhoff rods. Compared to prior works, the approach presented herein is not subject to the constant-curvature assumptions to derive the configuration space compliance, and we do not rely on computationally-expensive finite difference approximations to obtain the task space compliance. Using modal approximations over curvature space and Lie group integration, we obtain closed-form expressions for the task and configuration space compliance matrices of continuum robots, thereby bridging the gap between constant-curvature analytic formulations of configuration space compliance and variable curvature task space compliance. We first present an analytic expression for the compliance of a single Kirchhoff rod. We then extend this formulation for computing both the task space and configuration space compliance of a tendon-actuated continuum robot. We then use our formulation to study the tradeoffs between computation cost and modeling accuracy as well as the loss in accuracy from neglecting the Jacobian derivative term in the compliance model. Finally, we experimentally validate the model on a tendon-actuated continuum segment, demonstrating the model's ability to predict passive deflections with error below 11.5\% percent of total arc length.

==> format/preamble_algorithm.tex <==
\usepackage{algorithm,algorithmicx,algpseudocode}
%\usepackage{amssymb}

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}

\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]} 

%\algrenewcommand{\algorithmiccomment}[1]{\hfill$\blacktriangleright$ #1} %uncomment for black triangles

%%% example:
%\begin{algorithm}
%  \caption{Influx}
%  \label{influx}
%  \begin{algorithmic}[1]
%  \Input $p \in [0,1]$, $G$
%  \Output None \Comment{a test comment}
%  \For{$i = 0 \to 2^d-1$}\Comment{another test comment}
%    \If{$n(\nu_i) = 0$}
%      \If{ $x < p$}  \Comment{$x$ is a normal distribution number in the range of $[0,1]$}
%      \State Occupy $v_i$ site with probablility $p$
%      \EndIf
%    \EndIf
%  \EndFor
%  \end{algorithmic}
%\end{algorithm}

% for algorithmic package
%\renewcommand{\algorithmicxrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicxensure}{\textbf{Output:}}

